Definability equals recognizability for graphs of bounded treewidth

We prove a conjecture of Courcelle, which states that a graph property is definable in MSO with modular counting predicates on graphs of constant treewidth if, and only if it is recognizable in the following sense: constant-width tree decompositions of graphs satisfying the property can be recognized by tree automata. While the forward implication is a classic fact known as Courcelle's theorem, the converse direction remained open

==> prelims.tex <==
\begin{comment}

\subsection{Plan}

Stuff not to forget, in order not to make people angry:
\begin{itemize}
\item Hypergraph substitutions are used by Lapoire~\cite{Lapoire98}, who attributes this basic idea to Bauderon and Courcelle~\cite{BauderonC87}. Courcelle~\cite{Courcelle91a} also uses them, as he views tree decompositions as a hypergraph replacement grammar, where the graph is constructed by iteratively replacing hyperedges by hypergraphs of width $k$.
\item Understanding that one needs to MSO-define a decomposition is folklore, and it appears in all the papers above.
\item Courcelle~\cite{Courcelle91a} talks about {\em{strongly context-free}} graph languages (but it's impossible to understand anything from~\cite{Courcelle91a}), Lapoire~\cite{Lapoire98} calls it {\em{MSO-parsability}} after Courcelle~\cite{Courcelle91a}, and Jaffke and Bodlaender~\cite{JaffkeB15} explicitly develop a formalism of {\em{existentially MSOL-definable}}.
\item Jaffke and Bodlaender~\cite{JaffkeB15} encode the tree decomposition as a relational structure similarly to us.
\item The trick with guessing orientation by guessing a coloring was used by all the above works, see e.g. Lemma 4.8 in~\cite{Kaller00}.
\item We develop our own language to be self-contained.
\end{itemize}

\end{comment}

\begin{comment}
\subsection{Basic notation}

Unless otherwise stated, all graphs considered in this paper are finite, undirected, and simple; that is, they do not contain loops at vertices or parallel edges. 
For a graph $G$ and $X\subseteq V(G)$, by $G[X]$ we denote the subgraph induced by $X$ in $G$, and $G-X$ denotes $G[V(G)\setminus X]$. 

A hypergraph $H$ consists of its finite {\em{vertex set}} $V(H)$ and {\em{hyperedge set}} $E(H)$, where each element of $E(H)$, called a {\em{hyperedge}}, is a non-empty subset of $V(H)$. 
We allow multiple hyperedges consisting of exactly the same vertices; thus, by requiring that every hyperedge has cardinality $2$ we arrive at multigraphs without loops. 
For any $X\subseteq V(H)$, by $H[X]$ we denote the {\em{hypergraph induced by $X$}} defined as follows: 
the vertex set of $H[X]$ is $X$ and the hyperedge set is obtained from $E(H)$ by intersecting every hyperedge with $X$ and deleting all hyperedges that became empty in this manner. 
For a subset of hyperedges $F\subseteq E(H)$, by $H-F$ we denote the hypergraph obtained from $H$ by removing all hyperedges of $F$.

For a graph $G$ and a vertex subset $X\subseteq V(G)$, the {\em{torso}} of $G$ w.r.t. $X$ is a graph $\torso(G,X)$ on vertex set $X$, where an edge $uv$ is present if and only if it is present in $G[X]$, 
or there exists a path in $G$ that starts in $u$, ends in $v$, and whose internal vertices do not belong to $X$. 
Alternatively, $\torso(G,X)$ is obtained from $G[X]$ by turning the neighborhood in $X$ of each connected component of $G-X$ into a clique. 
The {\em{hypertorso}} of $G$ w.r.t. $X$ is a hypergraph $\hyptorso(G,X)$ on vertex set $X$ defined as follows: take $G[X]$, and for each connected component $C$ of $G-X$ introduce a hyperedge $N_G(V(C))$. 
Thus, $\torso(G,X)$ can be obtained from $\hyptorso(G,X)$ by turning every hyperedge into a clique.

For graphs $G_1,G_2$, by $G_1\dunion G_2$ we denote the disjoint union of $G_1$ and $G_2$.
\end{comment}

In this section we introduce additional notation for tree decompositions, and define sane tree decompositions that were already mentioned in the previous section.
Our notation largely follows Grohe and Marx~\cite{GroheM15}. Suppose $t$ is a tree decomposition of a graph $G$; then we denote the following sets for any node $x$ of $t$:
\begin{itemize}
\item The {\em{adhesion}} at $x$, denoted $\sep(x)$, is defined as $\bag(x)\cap \bag(y)$ where $y$ is the parent of $x$, or $\emptyset$ if $x$ is the root of $t$.
\item The {\em{cone}} at $x$, denoted $\cone(x)$, is defined as $\bigcup_{y\textrm{ is a descendant of }x}\, \bag(y)$.
\item The {\em{component}} at $x$, denoted $\comp(x)$, is defined as $\cone(x)\setminus \sep(x)$.
\end{itemize}
When $e=xy$ is an edge of decomposition $t$, we also can consider the {\em{adhesion at $e$}} defined as $\sep(e)=\bag(x)\cap \bag(y)$.

Operators $\bag(\cdot)$, $\sep(\cdot)$, $\cone(\cdot)$, and $\comp(\cdot)$ can be applied to any node in any tree decomposition. 
The result is always defined by the decomposition to which the node belongs, which will be always clear from the context.

In our proofs we often use a normalized form of tree decompositions, which we call {\em{sane}}.
Intuitively, sane decompositions are as fine as possible with respect to the connectivity of the graph.
We now recall the definition, which was already given in the previous section.

\begin{definition}\label{def:sane}
A rooted tree decomposition $t$ of a graph $G$ is called {\em{sane}} if the following conditions are satisfied:
\begin{enumerate}[(a)]
\item\label{p:notcontained} For each node $x$ of $t$, $\bag(x)\setminus \sep(x)\neq \emptyset$.
\item\label{p:connectivity} For each node $x$ of $t$, both $G[\cone(x)]$ and $G[\comp(x)]$ are connected.
\item\label{p:neighbors} For each node $x$ of $t$ and each $u\in \sep(x)$, $u$ has a neighbor in $\comp(x)$.
\end{enumerate}
\end{definition}

We remark that most approximation algorithms for treewidth produce tree decompositions that are sane. 
In fact, saneness often follows from explicit invariants maintained by the algorithm~\cite{BodlaenderDDFLP13,platypus}. 
The following lemma, which may be considered folklore, verifies that any tree decomposition can be conveniently sanitized.

\ifthenelse{\boolean{uglytwosided}}{

\begin{lemma}[\app]\label{lem:sanitation}
Suppose $t$ is a tree decomposition of a graph $G$. Then there exists a sane tree decomposition $s$ of $G$ where every bag in $s$ is a subset of some bag in $t$.
In particular, if $\tw(G)\leq k$ then $G$ admits a sane tree decomposition of width at most $k$.
\end{lemma}

}{

\begin{lemma}\label{lem:sanitation}
Suppose $t$ is a tree decomposition of a graph $G$. Then there exists a sane tree decomposition $s$ of $G$ where every bag in $s$ is a subset of some bag in $t$.
In particular, if $\tw(G)\leq k$ then $G$ admits a sane tree decomposition of width at most $k$.
\end{lemma}
\begin{proof}
For a tree decomposition $s$ of $G$, let $\Phi(s)=\sum_{x\in V(s)} |\comp(x)|^2$. 
Let $s$ be a tree decomposition of $G$ that is chosen as follows:
\begin{enumerate}[(i)]
\item\label{p:subset} Each bag of $s$ is a subset of some bag of $t$.
\item\label{p:potential} Among decompositions satisfying~\eqref{p:subset}, $s$ minimizes the potential $\Phi(s)$.
\item\label{p:tot-size}  Among decompositions satisfying~\eqref{p:subset} and~\eqref{p:potential}, $s$ has the minimum total size measured as $|V(s)|+|E(s)|+\sum_{x\in V(s)} |\bag(x)|$. 
\end{enumerate}
Decomposition $s$ is well defined due to $t$ satisfying property~\eqref{p:subset}. We now verify that $s$ is sane.

First, suppose that condition~\eqref{p:notcontained} is not satisfied for some node $x$. 
If $x$ has some parent $y$, then contracting edge $xy$ in $s$ and placing $\bag(y)$ at the node resulting from the contraction yields a tree decomposition $s'$ of $G$.
This tree decomposition has either strictly lower potential $\Phi(\cdot)$ (in case $\comp(x)\neq \emptyset$), or the same potential $\Phi(\cdot)$ but strictly smaller size. 
As the bags of $s'$ are a subfamily of the bags of $s$, this contradicts the choice of $s$. 
Also, if $x$ is the root in $s$ and $\bag(x)\setminus \sep(x)=\emptyset$, then in fact $\bag(x)=\emptyset$. 
Then we can remove $x$ from the decomposition and make its children roots of respective subtrees. 
This yields a tree decomposition of $G$ with the same bags, not larger potential $\Phi(\cdot)$, and strictly smaller size.

For condition~\eqref{p:connectivity}, we only verify the connectivity of $G[\comp(x)]$, because the connectivity of $G[\cone(x)]$ follows from the connectivity of $G[\comp(x)]$ and condition~\eqref{p:neighbors}. 
Suppose then that $G[\comp(x)]$ is not connected for some node $x$. 
This means that $\comp(x)$ can be partitioned into nonempty sets $A$ and $B$ with no edge between them in $G$. Obtain a tree decomposition $s'$ of $G$ as follows. 
Let $p$ be the subtree of $s$ rooted at $x$. 
Replace $p$ in $s$ by two copies $p_A$ and $p_B$ of $p$, where in $p_A$ every bag is replaced with its intersection with $A\cup \sep(x)$, and similarly for $p_B$. 
Since there is no edge in $G$ between $A$ and $B$, it is easy to verify that $s'$ obtained in this manner is indeed a tree decomposition of $G$. 
Moreover, if $y$ is a node of $p$, then the components at the copies of $y$ in $p_A$ and in $p_B$ form a partition of the component at $y$ in $p$.
By the convexity of function $a\to a^2$ we infer that $\Phi(s')$ is not larger than $\Phi(s)$. 
Moreover, the equality could hold only if for every node $y$ of $p$, the component at $y$ is being partitioned trivially: it is either entirely contained in $A$ or entirely contained in $B$. 
However, this is not the case for $y=x$, as both $A$ and $B$ are non-empty.
This implies that in fact $\Phi(s')<\Phi(s)$. 
As every bag of $s'$ is contained in a bag of $s$, which in turn is contained in a bag of $t$, this is a contradiction with the choice of $s$.

Finally, suppose that condition~\eqref{p:neighbors} is not satisfied for some node $x$ and some $u\in \sep(x)$. 
Since $\sep(x)\neq \emptyset$, $x$ has some parent $y$ and $u\in \bag(y)$. 
Obtain decomposition $s'$ by removing $u$ from every bag at every descendant of $x$, including $x$ itself. 
Since $u$ is still contained in $\bag(y)$, which in turn contains whole $\sep(x)$, and $u$ has no neighbors in $\comp(x)$, it follows that $s'$ is still a tree decomposition of $G$.
Moroever, it is easy to see that during the construction of $s'$, the component at each node could have only shrunk; hence, $\Phi(s')\leq \Phi(s)$.
Also $s'$ is obtained from $s$ by removing some vertices from some bags, so in particular the total size of $s'$ is strictly smaller than that of $s$. 
This is a contradiction with the choice of $s$.
\end{proof}

}

The next lemma gathers some basic properties of sane tree decompositions.
Their proofs follow very easily from the definition, and hence are omitted. 
In the sequel, we will often use these properties implicitly.

\begin{lemma}\label{lem:easy-sane}
Suppose $t$ is a sane tree decomposition of a graph $G$. Then:
\begin{enumerate}[(1)]
\item $t$ is a forest with one tree per each connected component of $G$.
\item The maximum size of a adhesion in $t$ is at most the width of $t$.
\item Suppose $s$ is a prefix of $t$ (i.e., a subforest closed under taking ancestors), and let $U_s$ comprise all the bags of all the nodes of $s$.
Then $\torso(G,U_s)$ can be obtained from $G[U_s]$ by turning $\sep(y)$ into a clique, for every node $y$ that is not in $s$, but whose parent is in $s$.
\item Sets $\bag(x)\setminus \sep(x)$, for nodes $x$ of $t$, form a partition of the vertex set of $G$.
\item\label{cnd:sane-int-parent} For every node $y$ of $t$ that has parent $x$, the set $\sep(y)$ contains at least one vertex of $\bag(x)\setminus \sep(x)$.
\end{enumerate}
\end{lemma}



